Initial State Interventions for Deconfounded Imitation Learning

Imitation learning suffers from causal confusion. This phenomenon occurs when learned policies attend to features that do not causally influence the expert actions but are instead spuriously correlated. Causally confused agents produce low open-loop supervised loss but poor closed-loop performance upon deployment. We consider the problem of masking observed confounders in a disentangled representation of the observation space. Our novel masking algorithm leverages the usual ability to intervene in the initial system state, avoiding any requirement involving expert querying, expert reward functions, or causal graph specification. Under certain assumptions, we theoretically prove that this algorithm is conservative in the sense that it does not incorrectly mask observations that causally influence the expert; furthermore, intervening on the initial state serves to strictly reduce excess conservatism. The masking algorithm is applied to behavior cloning for two illustrative control systems: CartPole and Reacher.

==> old.tex <==

Your goal is to simulate, as closely as possible, the usual appearance of typeset
 papers. This document provides an example of the desired layout and contains
 information regarding desktop publishing format, type sizes, and type faces.

\subsection{Full-Size Camera-Ready (CR) Copy}

If you have desktop publishing facilities, (the use of a computer to aid
 in the assembly of words and illustrations on pages) prepare your CR paper
  in full-size format, on paper 21.6 x 27.9 cm (8.5 x 11 in or 51 x 66 picas).
  It must be output on a printer (e.g., laser printer) having 300 dots/in, or
  better, resolution. Lesser quality printers, such as dot matrix printers,
   are not acceptable, as the manuscript will not reproduce the desired quality.

\subsubsection{Typefaces and Sizes:} There are many different typefaces and a large
variety of fonts (a complete set of characters in the same typeface, style,
 and size). Please use a proportional serif typeface such as Times Roman,
 or Dutch. If these are not available to you, use the closest typeface you
  can. The minimum typesize for the body of the text is 10 point. The minimum
  size for applications like table captions, footnotes, and text subscripts
  is 8 point. As an aid in gauging type size, 1 point is about 0.35 mm (1/72in).
   Examples are as follows:

\subsubsection{Format:} In formatting your original 8.5" x 11" page, set top and
bottom margins to 25 mm (1 in or 6 picas), and left and right margins
to about 18 mm (0.7 in or 4 picas). The column width is 88 mm (3.5 in or 21 picas).
 The space between the two columns is 5 mm(0.2 in or 1 pica). Paragraph
 indentation is about 3.5 mm (0.14 in or 1 pica). Left- and right-justify your
 columns. Cut A4 papers to 28 cm. Use either one or two spaces between sections,
 and between text and tables or figures, to adjust the column length.
  On the last page of your paper, try to adjust the lengths of the
  two-columns so that they are the same. Use automatic hyphenation and
   check spelling. Either digitize or paste your figures.

\begin{table}
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{UNITS}

Metric units are preferred for use in IEEE publications in light of their
international readership and the inherent convenience of these units in many fields.
In particular, the use of the International System of Units (SI Units) is advocated.
 This system includes a subsystem the MKSA units, which are based on the
 meter, kilogram, second, and ampere. British units may be used as secondary units
 (in parenthesis). An exception is when British units are used as identifiers in trade,
 such as, 3.5 inch disk drive.


\addtolength{\textheight}{-3cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ADDITIONAL REQUIREMENTS}

\subsection{Figures and Tables}

Position figures and tables at the tops and bottoms of columns.
Avoid placing them in the middle of columns. Large figures and tables
may span across both columns. Figure captions should be below the figures;
 table captions should be above the tables. Avoid placing figures and tables
  before their first mention in the text. Use the abbreviation ``Fig. 1'',
  even at the beginning of a sentence.
Figure axis labels are often a source of confusion.
Try to use words rather then symbols. As an example write the quantity ``Inductance",
 or ``Inductance L'', not just.
 Put units in parentheses. Do not label axes only with units.
 In the example, write ``Inductance (mH)'', or ``Inductance L (mH)'', not just ``mH''.
 Do not label axes with the ratio of quantities and units.
 For example, write ``Temperature (K)'', not ``Temperature/K''.

\subsection{Numbering}

Number reference citations consecutively in square brackets \cite{c1}.
 The sentence punctuation follows the brackets \cite{c2}.
 Refer simply to the reference number, as in \cite{c3}.
 Do not use ``ref. \cite{c3}'' or ``reference \cite{c3}''.
Number footnotes separately in superscripts\footnote{This is a footnote}
Place the actual footnote at the bottom of the column in which it is cited.
Do not put footnotes in the reference list.
Use letters for table footnotes (see Table I).

\subsection{Abbreviations and Acronyms}

Define abbreviations and acronyms the first time they are used in the text,
even after they have been defined in the abstract. Abbreviations such as
IEEE, SI, CGS, ac, dc, and rms do not have to be defined. Do not use
abbreviations in the title unless they are unavoidable.

\subsection{Equations}

Number equations consecutively with equation numbers in parentheses flush
 with the right margin, as in (1). To make your equations more compact
 you may use the solidus (/), the exp. function, or appropriate exponents.
  Italicize Roman symbols for quantities and variables, but not Greek symbols.
   Use a long dash rather then hyphen for a minus sign. Use parentheses to avoid
    ambiguities in the denominator.
Punctuate equations with commas or periods when they are part of a sentence:
$$\Gamma_2 a^2 + \Gamma_3 a^3 + \Gamma_4 a^4 + ... = \lambda \Lambda(x),$$
where $\lambda$ is an auxiliary parameter.

Be sure that the symbols in your equation have been defined before the
equation appears or immediately following.
Use ``(1),'' not ``Eq. (1)'' or ``Equation (1),''
except at the beginning of a sentence: ``Equation (1) is ...''.

   \begin{figure}[thpb]
      \centering
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{CONCLUSIONS AND FUTURE WORKS}

\subsection{Conclusions}

This is a repeat.
Position figures and tables at the tops and bottoms of columns.
Avoid placing them in the middle of columns. Large figures and tables
may span across both columns. Figure captions should be below the figures;
 table captions should be above the tables. Avoid placing figures and tables
  before their first mention in the text. Use the abbreviation ``Fig. 1'',
  even at the beginning of a sentence.
Figure axis labels are often a source of confusion.
Try to use words rather then symbols. As an example write the quantity ``Inductance",
 or ``Inductance L'', not just.
 Put units in parentheses. Do not label axes only with units.
 In the example, write ``Inductance (mH)'', or ``Inductance L (mH)'', not just ``mH''.
 Do not label axes with the ratio of quantities and units.
 For example, write ``Temperature (K)'', not ``Temperature/K''.


\subsection{Future Works}

This is a repeat.
Position figures and tables at the tops and bottoms of columns.
Avoid placing them in the middle of columns. Large figures and tables
may span across both columns. Figure captions should be below the figures;
 table captions should be above the tables. Avoid placing figures and tables
  before their first mention in the text. Use the abbreviation ``Fig. 1'',
  even at the beginning of a sentence.
Figure axis labels are often a source of confusion.
Try to use words rather then symbols. As an example write the quantity ``Inductance",
 or ``Inductance L'', not just.
 Put units in parentheses. Do not label axes only with units.
 In the example, write ``Inductance (mH)'', or ``Inductance L (mH)'', not just ``mH''.
 Do not label axes with the ratio of quantities and units.
 For example, write ``Temperature (K)'', not ``Temperature/K''.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ACKNOWLEDGMENTS}

The authors gratefully acknowledge the contribution of National Research Organization and reviewers' comments.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.

\begin{thebibliography}{99}

\bibitem{c1}
J.G.F. Francis, The QR Transformation I, {\it Comput. J.}, vol. 4, 1961, pp 265-271.

\bibitem{c2}
H. Kwakernaak and R. Sivan, {\it Modern Signals and Systems}, Prentice Hall, Englewood Cliffs, NJ; 1991.

\bibitem{c3}
D. Boley and R. Maier, "A Parallel QR Algorithm for the Non-Symmetric Eigenvalue Algorithm", {\it in Third SIAM Conference on Applied Linear Algebra}, Madison, WI, 1988, pp. A20.

\end{thebibliography}



==> related_works.tex <==
\section{RELATED WORKS}
\textbf{Imitation learning.}
Imitation learning is learning optimal control policies from the demonstrations from the expert policy executor, such as human expert \cite{schneider_analytic_2018}. Due to its advantage of removing the necessity for extensive interaction with the environment and delicate reward design, imitation learning have been widely used in reinforcement learning \cite{rashidinejad2021bridging, zhu2018reinforcement, sun2018truncated,DBLP:conf/cdc/CosnerYA22,DBLP:conf/cdc/StrongLB22,DBLP:conf/cdc/ZhangHLLZ21,DBLP:conf/cdc/GiammarinoP21,DBLP:conf/cdc/ChenPS021}. One of the major issues in imitation learning is the distributinoal shift problem where the learned policy shows unjustifiable behaviour due to encountering unseen stats during its execution. Existing works show that the distributional shift problem in imitation learning comes from causal misidentification or spurious causal relationship between the data and the policy \cite{de2019causal,DBLP:journals/corr/abs-2106-03443}. 

\textbf{Causal Inference.}
Causal Inference is the well-known problem that deduces the relationships between causes and effects among the variables \cite{DBLP:conf/cdc/Li021,DBLP:conf/cdc/XieKB020,DBLP:conf/cdc/PauliGBA21,DBLP:conf/cdc/ParkP22}. Most existing work take one of the approaches called ``causal discover'',
to find its relationship from recorded observations under some constraints \cite{https://doi.org/10.48550/arxiv.1605.08179,LouizosEtAl_arxiv17,Maathuis2010PredictingCE}.

Regarding with causal inference, one challenge in the imitation learning is confounding, which is also known as $\textit{causal delusion}$ \cite{de2019causal}. Namely, standard imitation learning does not assume the existence of latent variables that may affect the expert behavior but not captured by observations. Ortega et al.\cite{pedro2021CI} propose a interventional distribution in a causal structure model and claim that an imitator needs to refer the distribution during the policy learning. Tien et al. \cite{Tien2022} show a systematic study of causal confusion that learns the preference of reward functions which is provided by the human expert. Vuorio et al.\cite{Yuorio2022} propose learning a latent-conditional policy, where the environment dynamics is influnced by the latent variable. Pim de Haan et al. \cite{DBLP:journals/corr/abs-1905-11979} proposed causal graph parameterized policy learning that maps from multiple causal graphs to policies.

